Conditional independence testing: a predictive perspective

Conditional independence testing is a key problem required by many machine learning and statistics tools. In particular, it is one way of evaluating the usefulness of some features on a supervised prediction problem. We propose a novel conditional independence test in a predictive setting, and show that it achieves better power than competing approaches in several settings. Our approach consists in deriving a p-value using a permutation test where the predictive power using the unpermuted dataset is compared with the predictive power of using dataset where the feature(s) of interest are permuted. We conclude that the method achives sensible results on simulated and real datasets.

==> sections/05-theory.tex <==
\section{Theory}

Let $H_0$ denote the hypothesis that
$\Xop$ independent of $\Y$ given $\Xt$.
Similarly, let $\Hop$ denote that
$\Xop$ is independent of $(\Xt, \Y)$.
Figure \ref{fig:perm_diagram} illustrates that
$\Hop$ is a stronger hypothesis than $H_0$.
Since the permutation test samples from $\Hop$,
a typical permutation test might
not control the type I error whenever
$H_0$ holds but $\Hop$ does not.
The main challenge is to create
a special instance of the permutation test
which controls the type I error under $H_0$
even though it samples from $\Hop$.

\begin{figure}[!htb]
 \centering
 \begin{minipage}{0.45\textwidth}
  \centering
  \indephz
  \caption{Joint distribution under $H_0$.}
 \end{minipage}\hfill
 \begin{minipage}{0.45\textwidth}
  \centering
  \indepperm
  \caption{Joint distribution under permutation.}
  \label{fig:perm_diagram}
 \end{minipage}
\end{figure}


==> tab_hiptest_null.tex <==
\begin{table}[htpb]
\caption{Test of uniformity of the observed p-values for each simulation study configuration. Configurations for which the p-value was approximately zero have been omitted.}
\label{tab:hiptest_null}
\centering
\begin{tabular}{|Hlllccc|}
\hline
{} &  method & retrain & db size & estimator & distribution &  pvalue \\ \hline
0  &  permutation &                 True &    1000 &       ann &            0 &    0.33 \\
1  &  permutation &                 True &   10000 &       ann &            0 &    0.46 \\
2  &  permutation &                False &    1000 &       ann &            0 &    0.19 \\
3  &  permutation &                False &   10000 &       ann &            0 &    0.48 \\
4  &  permutation &                 True &    1000 &        rf &            0 &    0.05 \\
5  &  permutation &                 True &   10000 &        rf &            0 &    0.39 \\
6  &  permutation &                False &    1000 &        rf &            0 &    0.56 \\
7  &  permutation &                False &   10000 &        rf &            0 &    0.24 \\
8  &  permutation &                 True &    1000 &    linear &            0 &    0.18 \\
9  &  permutation &                 True &   10000 &    linear &            0 &    0.71 \\
10 &  permutation &                False &    1000 &    linear &            0 &    0.97 \\
11 &  permutation &                False &   10000 &    linear &            0 &    0.36 \\
12 &  permutation &                 True &    1000 &       ann &            1 &    0.52 \\
13 &  permutation &                 True &   10000 &       ann &            1 &    0.45 \\
14 &  permutation &                False &    1000 &       ann &            1 &    0.61 \\
15 &  permutation &                False &   10000 &       ann &            1 &    0.95 \\
16 &  permutation &                 True &    1000 &        rf &            1 &    0.02 \\
17 &  permutation &                 True &   10000 &        rf &            1 &    0.48 \\
18 &  permutation &                False &    1000 &        rf &            1 &    0.19 \\
19 &  permutation &                False &   10000 &        rf &            1 &    0.44 \\
20 &  permutation &                 True &    1000 &    linear &            1 &    0.96 \\
21 &  permutation &                 True &   10000 &    linear &            1 &    0.25 \\
22 &  permutation &                False &    1000 &    linear &            1 &    0.38 \\
23 &  permutation &                False &   10000 &    linear &            1 &    0.74 \\
24 &  permutation &                 True &   10000 &       ann &            2 &    0.62 \\
25 &  permutation &                 True &    1000 &        rf &            2 &    0.55 \\
26 &  permutation &                 True &   10000 &        rf &            2 &    0.30 \\
27 &  permutation &                 True &    1000 &    linear &            2 &    0.18 \\
28 &  permutation &                 True &   10000 &    linear &            2 &    0.94 \\
29 &  permutation &                 True &    1000 &       ann &            3 &    0.01 \\
30 &  permutation &                 True &   10000 &       ann &            3 &    0.57 \\
\hline
\end{tabular}
\end{table}
